Detectability of the $\tau_{es}$-21cm cross-correlation: a tomographic probe of patchy reionization

The cross-correlation between fluctuations in the electron scattering optical depth $\tau_{\rm es}$ as probed by future Cosmic Microwave Background (CMB) experiments, and fluctuations in the 21cm differential brightness temperature $\Delta T_{\rm 21cm}$ as probed by ground-based radio interferometers, will trace the reionization history of the Universe. In particular, the $\tau_{\rm es}-$21cm cross-correlation should yield a determination of the characteristic bubble size distribution and ionization fraction as a function of redshift. When assuming that the cross-correlation signal is limited by instrumental noise rather than by foregrounds, we estimate its potential detectability by upcoming experiments. Specifically, the combination of HERA and Simons Observatory, CMB-S4 and PICO should yield a signal-to-noise ratio around 3 - 6, while and the exploitation of the SKA should increase it to 10-20. Finally, we have discussed how such levels of detectability can be affected when (simply modeled) 21cm foregrounds are present. For the most promising PICO$\times$SKA configuration, an efficiency of foreground removal to a level of $7\times 10^{-4}$ is needed to achieve a $5\sigma$ detection of the cross-correlation signal; in addition, safe avoidance of foreground contamination in the line-of-sight Fourier modes above $0.03 \,h\,\rm Mpc^{-1}$ would guarantee a detection significance around $3\sigma$.

==> section_andrea.tex <==
In this paper, we assume the \citet{Mancuso2016a, Mancuso2016b} and \citet{Lapi2017} models of cosmological star formation history.  These are based on analyses of recent dust-corrected UV, far-IR and radio data (see figure ~\ref{fig|SFR_func}).


For galaxies with relatively low star formation rates ($\dot M_\star\lesssim 30\, M_{\odot}$ yr$^{-1}$), UV observations are the most important tracers of the SFR.  Dust emission is mainly due to the diffuse (cirrus) dust component and attenuation is mild. Thus UV data extending down to a magnitude $M_{\rm UV}\approx -17$ have been dust-corrected according to the local empirical relation between the UV slope $\beta_{\rm UV}$ and the IR-to-UV luminosity ratio IRX \citep[see][]{Meurer1999}, that is also routinely exploited for high-redshift galaxies \citep[see][]{Bouwens2009, Bouwens2015, Bouwens2016, Bouwens2017}. A Meurer/Calzetti prescription has been adopted, but the determination of the SFR functions is only marginally affected at the faint end by choosing a different extinction law, like for example the Small Magellanic Cloud (SMC) one.

For galaxies with relatively higher star formation rates, far-IR and radio data are the most important tracers as dust emission is largely dominated by molecular clouds and the UV dust corrections are large and uncertain \citep[see][]{Silva1998, Efstathiou2000, Coppin2015, Reddy2015, Fudamoto2017}. Interestingly, the shape of the SFR function for $\dot M_\star\gtrsim 10^2\, M_\odot$ yr$^{-1}$, which so far has been probed only indirectly at $z\gtrsim 4$ due to sensitivity limits in current far-IR surveys, is found to agree out to $z\lesssim 6$ with the constraints from the recent VLA-COSMOS radio survey \citep[see][]{Novak2017} and from the few individual galaxies detected at $z\gtrsim 5$ with ALMA and SMA \citep[see][]{Riechers2017, Zavala2017}.

The luminosity $L$ has been converted into the SFR $\dot M_\star$ using $\log {\dot M_\star/ M_\odot~{\rm yr}^{-1}} \approx -9.8+\log {L/ L_\odot}$, a good approximation both for far-IR and (intrinsic) UV luminosities, as expected on energy conservation arguments, under the assumption of a Chabrier's IMF. Note that actually this conversion factor depends on the star formation history, and specifically on duration and age of the burst \citep[see][]{Efstathiou2000, Bressan2002}; the standard value adopted here is the average for a continuous star formation over $100$ Myr, the age at which $90\%$ of emission has been contributed \citep[see][their table 1]{Kennicutt2012}.

The SFR function can be described as a smooth Schechter function
\begin{equation}
{{\rm d}N\over {\rm d}\log\dot M_\star}(\dot M_\star,z) = \mathcal{N}(z)\, \left[\dot M_\star\over\dot M_{\star, c}(z)\right]^{1-\alpha(z)}\,e^{-\dot M_\star/\dot M_{\star, c}(z)}~,
\end{equation}
with three parameters: the overall normalization $\mathcal{N}$, the characteristic SFR $\dot M_{\star, c}$ and the faint end slope $\alpha$. The redshift evolution for each parameter $p(z)$ of the Schechter function has been described as a third-order polynomial in log-redshift $p(z)=p_0+p_1\, \xi+p_2\,\xi^2+p_3\,\xi^3$, with $\xi=\log(1+z)$. The values of the parameters $\left\{p_i\right\}$ are reported in Table~1 of \citet{Lapi2017}. In Figure~\ref{fig|SFR_func} dashed lines refer to the (dust-corrected) UV-inferred SFR functions while solid line to the global (UV+far-IR/radio) SFR functions. The behavior of the normalization $\mathcal{N}$ and of the characteristic SFR $\dot M_{\star, c}$ highlights that UV surveys tend to pick up many galaxies with low SFR, while far-IR surveys also select less numerous galaxies with higher SFR; this mirrors the fact that high SFRs are usually associated to large dust abundance. The evolution with redshift of these parameters shows that most of the SFR occurs in dusty galaxies around redshift $z\approx 2$ (cf. also Figure~\ref{fig|SFR_cosm}); on the other hand, toward high redshift $z\gtrsim 6$ the dust content progressively decreases and UV surveys become more effective in selecting the typical population of star forming galaxies. For the purpose of this paper, the high-redshift evolution is most relevant.

\citet{Mancuso2016a, Mancuso2016b} and \citet{Lapi2017} validate the SFR functions against independent datasets, including integrated galaxy number counts at significative far-IR/(sub)mm/radio wavelengths, counts/redshift distributions of strongly gravitationally-lensed galaxies, stellar mass function via the continuity equation, main sequence of star-forming galaxies, and even associated AGN statistics. In particular, the analysis of the main sequence for high-redshift galaxies and AGNs presented in \citet{Mancuso2017} and Lapi et al. (2017b) highlights that the current data can be consistently interpreted in terms of an in situ coevolution scenario for star formation and black hole accretion, envisaging these as local, time coordinated processes.

Since faint galaxies are likely the source of much of the ionizing background, we need to extrapolate the SFR to well beyond the magnitude limit of the current blank field surveys $M_{\rm UV}\approx -17$ (corresponding to SFR $\dot M_\star\approx$ a few $10^{-1}\, M_\odot$ yr$^{-1}$) down to $M_{\rm UV} \approx -13$  (corresponding to SFR $\dot M_\star\approx$ a few $10^{-2}\, M_\odot$ yr$^{-1}$). Actually, at redshifts $z\lesssim 6$ the faint end of the luminosity/SFR functions has been recently explored, though still with large uncertainties, even down to $M_{\rm UV} \approx -13$ via gravitational lensing by foreground galaxy clusters  \citep[see][]{Alavi2014, Alavi2016, Livermore2017, Bouwens2016}. We have reported (but not used in the fit because of the still large systematic uncertainties) these data in Figure~\ref{fig|SFR_func} to highlight that they are indeed consistent with the extrapolation of our SFR functions; specifically, the faint portion of the SFR function is seen to keep rising steeply with $\alpha\lesssim 2$ out to $z\lesssim 6$.

\subsection{Cosmic star formation rate density}\label{sec|SFR_cosm}

Based on the star formation rate functions in the previous section, we can compute a star formation rate density:
\begin{equation}\label{eq|SFR_func}
\rho_{\rm SFR}(z) = \int_{\dot M_\star^{\rm min}}^\infty{\rm d}\log \dot M_{\star}\, {{\rm d}N\over {\rm d}\log \dot M_\star}\, \dot M_\star~;
\end{equation}
Since the SFR function diverges at the faint end ($\alpha\gtrsim 1$), the results are sensitive to the minimum SFR cutoff, $\dot M_\star^{\rm min}$.  Figure \ref{fig|SFR_cosm} shows the cosmic star formation rate based on integrating the UV-corrected SFR to three cut-offs: $M_{\rm UV}\approx -17$, the observational limit of current blank field surveys. The outcome matches the determination by \citet[][dotted line]{Madau2014} and is in good agreement with the dust corrected data by \citet[][cyan shaded area]{Schiminovich2005} at $z\lesssim 4$ and by \citet[][cyan squares]{Bouwens2015} at $z\gtrsim 4$. On the other hand, the cosmic SFR density from (dust-corrected) UV data is inconsistent with other datasets both at low and high redshift. Specifically, at redshift $z\lesssim 4$ it falls short with respect to the multiwavelength determination by \citet[][orange shaded area]{Hopkins2006} based on UV/optical, radio, H$\alpha$ and mid-IR $24\, \mu$m data, to the far-IR measurements from \textsl{Herschel} by \citet{Magnelli2013} and \citet[][red shaded area]{Gruppioni2013}, and by the recent estimate from deblended data from \textsl{Herschel}, JCMT/AzTEC and JCMT/SCUBA-2 in the GOODS field by \citet{Liu2017}. At redshift $z\gtrsim 4$ it underestimates the determinations based on stacking of far-IR data from \textsl{Herschel} by \citet[][red dots]{Rowan2016}, the measurements from radio data by \citet{Novak2017}, and the estimates based on long GRB rates from \textsl{Swift} by \citet{Kistler2009, Kistler2013}. This mostly reflects the fact, already mentioned above, that the UV-inferred SFR functions (even corrected for dust extinction by the UV slope) appreciably underestimate the number density of dusty galaxies with $\dot M_\star\gtrsim 30\, M_\odot$ yr$^{-1}$.

Then we compute the cosmic SFR density exploiting our global SFR functions down to the same magnitude limit $M_{\rm UV}^{\rm min}\approx -17$. The outcome (solid line) is found to be in good agreement both with the \citet{Hopkins2006}, \citet{Gruppioni2013} and \citet{Liu2017} determinations at $z\lesssim 4$, with the stacked far-IR data by \citet{Rowan2016} at $z\gtrsim 4$. In Figure \ref{fig|SFR_cosm} we also show the outcomes when integrating our global SFR functions down to $M_{\rm UV}^{\rm lim}\approx -13$ (dot-dashed line) and $-12$ (dashed line); as we shall discuss in the next Section, these value are suggested by the recent data on the reionization history of the Universe in terms of electron scattering optical depth $\tau_{\rm es}\approx 0.058$ as measured by \citet{Planckxlvii}.

\subsection{Reionization history}\label{sec|reion}
The cosmic star formation history determines the cosmic ionization history.  The cosmic ionization rate is proportional to cosmic SFR density:
\begin{equation}
\dot N_{\rm ion}\approx f_{\rm esc}\, k_{\rm ion}\, \rho_{\rm SFR}~;
\end{equation}
here $k_{\rm ion}\approx 4\times 10^{53}$ is the number of ionizing photons s$^{-1}$ $(M_\odot/\rm yr)^{-1}$, with the quoted value appropriate for a Chabrier IMF, and $f_{\rm esc}\approx 1-20 \%$ is the poorly constrained average escape fraction for ionizing photons from the interstellar medium of high-redshift galaxies \citep[see][]{Mao2007, Dunlop2013, Robertson2015}. Note that two other parameters implicitly entering in the expression $\rho_{\rm SFR}$ are the minimum UV limiting magnitude, and the faint-end slope of the SFR functions $\alpha$ discussed at the end of Section ~\ref{sec|SFR_func}.

The competition between ionization and recombination determines the evolution of the ionization state of the universe \citep[see][]{Madau1999, Ferrara2014}:
\begin{equation}
\dot Q_{\rm HII} = {\dot N_{\rm ion}\over \bar n_{\rm H}}-{Q_{\rm HII}\over
t_{\rm rec}}
\label{ionfrac}
\end{equation}
Here $\bar n_{\rm H}\approx 2\times 10^{-7}\, (\Omega_b h^2/0.022)$ cm$^{-3}$ is the mean comoving hydrogen number density. In addition, the recombination timescale reads $t_{\rm rec}\approx 3.2$ Gyr $[(1+z)/7]^{-3}\, C_{\rm HII}^{-1}$, where the case B coefficient for an IGM temperature of $2\times 10^4$ K has been used; this timescale crucially depends on the clumping factor of the ionized hydrogen, for which a fiducial value $C_{\rm HII}\approx 3$ is usually adopted \citep[see][]{Pawlik2013}.

The electron scattering optical depth is proportional to the integrated electron density along the line-of-sight:
\begin{equation}\label{eq_tau_eerm}
\tau_{\rm es}(z) = c\, \sigma_{\rm T}\,\bar n_{\rm H}\int_t^{t_0}{\rm d}t'\,f_e\,Q_{\rm HII}(z')(1+z')^2 ;
\end{equation}
here $dt=\frac{dz}{H(z)}$ and $H(z)=H_0\,[\Omega_M\,(1+z)^3+1-\Omega_M]^{1/2}$ is the Hubble
parameter, $c$ is the speed of light, $\sigma_{\rm T}$ the Thomson cross
section and $f_e$ the number of free-electrons per ionized hydrogen atom (assuming double
Helium ionization at $z\lesssim 4$.).

Figure~\ref{fig|reion} shows the cosmic reionization history computed from our global SFR function integrated down to different $M_{\rm UV}^{\rm lim}$, on assuming a conservative value $f_{\rm esc}\approx 0.1$ for the escape fraction of ionizing photons. When adopting $M_{\rm UV}^{\rm lim}\approx -13$, the outcome (black dot-dashed line) agrees with the value of the optical depth for electron scattering $\tau_{\rm }\approx 0.058$ recently measured by the \textsl{Planck} mission. For reference, the dotted line represents the optical depth expected in a fully ionized Universe up to redshift $z$; this is to show that the bulk of the reionization process occurred at $z \sim 8-9$ and was almost completed at $z \sim 6$ \citep[see][]{Schultz2014}. Note that from this perspective, the detailed behavior of the SFR functions at $z\lesssim 6$ and at $z\gtrsim 10$, and the related ionizing background, are only marginally relevant. Remarkably, the evolution of the ionized fraction $Q_{\rm HII}$ illustrated in the inset is fully consistent with upper and lower limits from the plethora of independent observations collected by \citep{Robertson2015}.

When adopting $M_{\rm UV}^{\rm lim}\approx -17$, that corresponds to the observational limits of current blank-field UV surveys at $z\gtrsim 6$ (cf. Figure\ref{fig|SFR_cosm}), the outcome on the optical depth (black solid line) touches the lower boundary of the 1$\sigma$ region allowed by \textsl{Planck} data, and the evolution of the $Q_{\rm HII}$ parameter is inconsistent with the aforementioned observational limits. At the other end, going much beyond $M_{\rm UV}^{\rm lim}\approx -13$ is not allowed, since already for $M_{\rm UV}^{\rm lim}\approx -12$ the resulting optical depth (black dashed line) touches the upper boundary of the 1$\sigma$ region from \textsl{Planck} data.

Note that these outcomes suffer to some extent of parameter degeneracy, as highlighted by the expression
\begin{equation}
f_{\rm esc}\, k_{\rm ion}\,C_{\rm HII}^{-0.3}\, \Gamma[2-\alpha;\dot M_\star^{\rm lim}/\dot M_{\star,c}]\approx {\rm const},
\end{equation}
where $\Gamma[a;z]\equiv \int_z^\infty{\rm
d}x~x^{a-1}\,e^{-x}$ is the incomplete $\Gamma-$function; the parameters involved are the escape fraction $f_{\rm esc}$, the ionizing rate per unit SFR $k_{\rm ion}$ associated mainly to the IMF, the clumping factor $C_{\rm HII}$, the faint-end slope of the SFR function $\alpha$, and the UV magnitude limit $M_{\rm UV}^{\rm lim}$. The strongest dependencies are on $f_{\rm esc}$ and on the limiting magnitude $M_{\rm UV}^{\rm lim}$. For example, to reproduce the \textsl{Planck} best estimate $\tau_{\rm es}\approx 0.058$ for $M_{\rm UV}^{\rm lim}\approx -17$, it would be necessary to force $f_{\rm esc}$ to implausible values $\gtrsim 0.2$; at the other end, setting $M_{\rm UV}^{\rm lim}\approx -12$ would require $f_{\rm esc}\lesssim 0.05$, but at the cost of worsening the agreement with the observational constraints on $Q_{\rm HII}$.

Thus the combined constraints on the cosmic reionization history from Planck and the cosmic SFR density measured at high redshifts $z\gtrsim 6$ from galaxy surveys (see Figure \ref{fig|SFR_cosm}) point toward a limiting UV magnitude  $M_{\rm UV}^{\rm lim}\approx -13$ and to an escape fraction $f_{\rm esc}\approx 10 \%$.

\begin{figure}[t]
\begin{center}
\includegraphics[width=1\textwidth]{Figures/SFR_func_anirban.eps}
\caption{The SFR functions at redshifts $z = 0$ (green), $1$ (red), $3$ (orange), $6$ (cyan), and $8$ (blue) determined according to the procedure by \citep{Mancuso2016a, Mancuso2016b, Mancuso2017} and \citep{Lapi2017}. Solid lines refer to the rendition from UV (dust corrected according to standard prescriptions based on the UV slope) plus far-IR/radio data; dotted lines refer to the rendition from only (dust-corrected) UV data. UV data (open symbols) are from \citet[diamonds]{Vanderburg2010}, \citet[pentagons]{Bouwens2015}, \citet[][inverse triangles]{Finkelstein2015}, \citet[][triangles]{Cucciati2012}, \citet[][spirals]{Wyder2005}, \citet[][crosses]{Oesch2010}, \citet[][asterisks]{Alavi2016}, \citet[][plus signs]{Bouwens2016}; far-IR data from \citet[][hexagons]{Gruppioni2015}, \citet[][circles]{Magnelli2013}, \citet[][squares]{Gruppioni2013}, \citet[][stars]{Lapi2017}, and \citet[][pacmans]{Cooray2014}; radio data from \citet[][clovers]{Novak2017}.}
\label{fig|SFR_func}
\end{center}
\end{figure}


\begin{figure}[t]
\begin{center}
\includegraphics[width=1\textwidth]{Figures/SFR_cosm_anirban.eps}
\caption{Cosmic SFR density as a function of redshift. The solid, dot-dashed, and dashed lines are our results on using the SFR functions from UV+far-IR/radio data presented in Figure~\ref{fig|SFR_func}, integrated down to a magnitude limit $M_{\rm UV}\lesssim -17$, $-13$, and $-12$, respectively. For comparison, the dotted line illustrates the determination by \citet{Madau2014} from dust-corrected UV data integrated down to a magnitude limit $M_{\rm UV}\lesssim -17$. At $z\lesssim 4$ data are from (dust-corrected) UV observations by \citet[][cyan shaded area]{Schiminovich2005}; far-IR observations by \citet[][magenta shaded area]{Gruppioni2013}; multiwavelength determination including UV, radio, H$\alpha$, and mid-IR 24 $\mu$m data collected by \citet[][orange shaded area]{Hopkins2006}; deblended far-IR/sub-mm data on the GOODS field by Liu et al. (2017; red stars). At higher redshifts $z \gtrsim 4$, we report the estimate of the SFR density inferred from (dust-corrected) UV data by \citet[][cyan sqares]{Bouwens2015}, stacked IR data by \citet[][magenta circles]{Rowan2016}, and long GRB rates by \citet[][green stars]{Kistler2009, Kistler2013}.}
\label{fig|SFR_cosm}
\end{center}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=1\textwidth]{Figures/reion_anirban.eps}
\caption{Reionization history of the universe, in terms of the redshift
evolution of the optical depth $\tau_{\rm es}$ for electron scattering. Solid, dot-dashed and dashed lines illustrate the outcomes from our SFR functions integrated down to UV-magnitude limits $M_{\rm UV}\lesssim -17$, $-13$, and $-12$, respectively for an escape fraction of ionizing photons $f_{\rm esc}\approx 0.1$. For reference, the dotted line refers to a fully ionized universe up to redshift $z$. The green line shows the measurement (with the $1\sigma$ and $2\sigma$ uncertainty regions highlighted by the dark and light green areas respectively) from \citet{Planckxlvii}. In the inset, the corresponding evolution of the ionized fraction $Q_{\rm HII}$ is plotted, together with upper and lower limits from various observations collected by \citet[][empty circles]{Robertson2015}.}\label{fig|reion}
\end{center}
\end{figure}
\clearpage
